Structure of Heavy Nuclei Based on Nucleon Quartets

Several topics concerning nuclear structure and electromagnetic interactions of heavy nuclei are reviewed. These comprehend the deformed single-particle shell model, nuclear collective motion, symmetry breaking and approximate symmetry restoring in atomic nuclei, particularly the proxy-SU(3) scheme. The relations between these theoretical frameworks are stated and it is shown how they contribute to a better and broader understanding of atomic nuclei. The semi-microscopic algebraic quartet model of atomic nuclei in the proxy-SU(3) scheme is applied to obtain previously unknown irreducible representations, deformation parameters, nuclear excited states and electromagnetic transition probabilities for certain heavy isotopes. The experimental data available for such nuclear region is currently very poor, so in preparation for future experimental efforts the theoretical background is developed along with some perspectives to work on are proposed.

==> abbreviations.tex <==
\begin{tabbing}
  aaaaaaaaaaaaaaaaa \= aaaaaaaaaaaaaaaaaaaaaa\kill\abbrev{BAO}{Baryon acoustic oscillation}
    
                                                     

\end{tabbing}

==> lagrangian-T13A.tex <==
\section{The model}
 The particle content consist of two $SU(2)_L$-doublets vector-like
 Weyl fermions of opposite hypercharges $\eta_u$, $\eta_d$; one singlet
 Weyl fermion of zero hypercharge $N$, and three of singlet real
 scalars of zero hypercharges. All of them odd under some $Z_2$
 symmetry.

\section{Preliminars}

Weyl spinors tranform under Lorentz as shown in Table~\ref{tab:electron}, illustrated for the case of the electron.

\begin{table}
  \centering
  \begin{tabular}{llll}
    Name & Symbol & Lorentz & $U(1)_Q$\\\hline
   $e_L^-$: left electron & $\xi_{\alpha}$ & ${M_{\alpha}}^{\beta}$ & $e^{i\theta}$\\
   $\left( e_L^- \right)^{\dagger}$: right positron    & $\left( \xi_{\alpha} \right)^{\dagger}=\xi^{\dagger}_{\dot{\alpha}}$ & ${{M^{*}}_{\dot{\alpha}}}^{\dot{\beta}}$ & $e^{-i\theta}$\\
   $e_R$: right electron   & $\left( \eta^{\alpha} \right)^{\dagger}=\eta^{\dagger\;\dot{\alpha}}$ & ${\left[ \left( M^{-1} \right)^\dagger \right]^{\dot{\alpha}}}_{\dot{\beta}}$& $e^{i\theta}$\\
   $\left( e_R^{-} \right)^{\dagger}$: left positron &$\eta^{\alpha}$& ${\left[ \left( M^{-1} \right)^T \right]^{\alpha}}_{\beta}$ & $e^{-i\theta}$\\\hline
  \end{tabular}
  \caption{Electron components}
  \label{tab:electron}
\end{table}



\section{Weyl spinors}
Consider the following set of Weyl spinor
\begin{align*}
  L=&
  \begin{pmatrix}
  \xi_{1\alpha}\\
  \xi_{2\alpha}
  \end{pmatrix}
  =
  \begin{pmatrix}
  \nu_L\\
  e_L    
  \end{pmatrix}&
  N=&\eta_1^{\alpha} \nonumber\\
  R_u=&
  \begin{pmatrix}
  \eta_2^{\dagger\dot{\alpha}}\\
  \eta_3^{\dagger\dot{\alpha}}\\
  \end{pmatrix}
  =
  \begin{pmatrix}
   \psi_R^0\\
   \psi_R^-    
  \end{pmatrix}&R_d=&
  \begin{pmatrix}
       \xi_{3\alpha}\\
       \xi_{4\alpha}
  \end{pmatrix}=
  \begin{pmatrix}
      \psi_L^0\\
      \psi_L^-    
  \end{pmatrix}
.\end{align*}
In order to have all the new fields in term of Weyl \emph{left}-fermions, it is convinient to define (the $\dagger$ for Weyl spinors just stands for conjugate)  
\begin{align}
  \widetilde{R}_u= i\sigma_2 R_u^{\dagger}=&i
  \begin{pmatrix}
    0 &-i\\
    i & 0\\
  \end{pmatrix}\begin{pmatrix}
  \eta_2^{\dagger\dot{\alpha}}\\
  \eta_3^{\dagger\dot{\alpha}}\\
  \end{pmatrix}^{\dagger}\nonumber\\
=&
  \begin{pmatrix}
    0 &1\\
    -1 & 0\\
  \end{pmatrix}  \begin{pmatrix}
 \left(   \eta_2^{\dagger\dot{\alpha}} \right)^{\dagger}\\
  \left( \eta_3^{\dagger\dot{\alpha}} \right)^{\dagger}\\
  \end{pmatrix}\nonumber\\
=&\begin{pmatrix}
  \eta_3^{\alpha}\\
  -\eta_2^\alpha\\
  \end{pmatrix}.
 \end{align}


A $SU(2)$-doublet of vector-like fermions can be written in terms
\emph{two} $SU(2)$-doublets of Weyl left-fermions with opposite
hypercharges, $Y=-1/2$ and $Y=+1/2$, as
\begin{align*}
  \widetilde{R}_{u}=&\begin{pmatrix}
\widetilde{R}_{u}^+\\    
\widetilde{R}_{u}^0
  \end{pmatrix}=
  \begin{pmatrix}
    \left( \psi_{R}^{-} \right)^{\dagger}\\
    -{\psi_{R}^{0}}^{\dagger}
  \end{pmatrix}
&  R_{d}=&\begin{pmatrix}
R_{d}^0\\    
R_{d}^-
  \end{pmatrix}=
  \begin{pmatrix}
    \psi_{L}^{0}\\
    \psi_{L}^{-}
  \end{pmatrix}
\end{align*}
Following the usual convention to contract the index
\begin{align}
  {}_{\alpha}\ {}^{\alpha} \qquad {}^{\dot{\alpha}}\ {}_{\dot{\alpha}}\;,
\end{align}
the Lagrangian is
\begin{align}
\label{eq:lt13aib}
  -\mathcal{L}=&M_D \epsilon_{ab}R^a_d \widetilde{R}^b_u+\tfrac{1}{2}M_N NN-h'_{i\alpha} \epsilon_{ab}\widetilde{R}_u^a L_{i}^b S'_{\alpha}-\lambda_d\, \epsilon_{ab}H^a R_d^b N-\lambda_u \epsilon_{ab}\widetilde{H}^a \widetilde{R}_u^b N+\text{h.c}\nonumber\\
&-\left[ \mu^2 \epsilon_{ab}\widetilde{H}^{a}H^b+\tfrac{1}{2}\lambda_1 \left( \epsilon_{ab} \widetilde{H}^{a}H^b\right)^2+\tfrac{1}{2}\left({M'}_S^2\right)_{\alpha\beta} S'_{\alpha}S'_\beta
   +\lambda^{\prime SH}_{\alpha\beta} \epsilon_{ab}\widetilde{H}^{a}H^bS'_{\alpha}S'_{\beta}+\lambda^{\prime S}_{\alpha\beta\gamma\delta}S'_{\alpha}S'_{\beta}S'_{\gamma}S'_{\delta}  \right]
\end{align}
where
\begin{align*}
  {H}=&  \begin{pmatrix}
    H^+ \\ H^0
  \end{pmatrix}&
  \widetilde{H}=&  \begin{pmatrix}
    {H^0}^{*} \\ -H^-
  \end{pmatrix}
\end{align*}
Note that a term like $\epsilon_{ab}\widetilde{R}_d^a L^b$ have the wrong Lorentz sctructure $\xi_{\dot{\alpha}}^{\dagger}\xi_{\alpha}$. 

For the $Z_2$--odd scalars we have in the basis
$
  \mathbf{S}=
  \begin{pmatrix}
    S_1&
    S_2&
    \cdots&
    S_{\alpha}
  \end{pmatrix}^{\operatorname{T}}
$, where now $\alpha,\beta$ is the number of real scalar fields
\begin{align*}
    \mathcal{L}_S=&\frac{1}{2}{\mathbf{S}'}^{\operatorname{T}}{\mathbf{M}'}_S^2\mathbf{S}'
+ \epsilon_{ab}\widetilde{H}^a H^b {\mathbf{S}'}^{\operatorname{T}}\boldsymbol{\lambda}^{\prime SH}\mathbf{S}' 
+ S'_{\gamma}\left( {\mathbf{S}'}^{\operatorname{T}}\boldsymbol{\lambda}^{\prime S}\mathbf{S}' \right)_{\gamma\delta} S'_{\delta} \nonumber\\
=&\frac{1}{2}{\mathbf{S}'}^{\operatorname{T}}{\mathbf{M}'}_S^2\mathbf{S}'
+ \epsilon_{ab}\widetilde{H}^a H^b {\mathbf{S}'}^{\operatorname{T}}\boldsymbol{\lambda}^{\prime SH}\mathbf{S}' 
+ \mathbf{S'}^{\operatorname{T}}\left( {\mathbf{S}'}^{\operatorname{T}}\boldsymbol{\lambda}^{\prime S}\mathbf{S}' \right)\mathbf{S'} \,,
\end{align*}


After the spontaneous symmetry breaking
\begin{align}
  \mathcal{L}_S\supset&\frac{1}{2}{\mathbf{S}'}^{\operatorname{T}}{\boldsymbol{\mathcal{M}}'}_S^2\mathbf{S}' \nonumber\\
=&\frac{1}{2}{\mathbf{S}}^{\operatorname{T}}\left( \mathbf{R}^T{\boldsymbol{\mathcal{M}}'}_S^2\mathbf{R} \right)\mathbf{S} \nonumber\\
=&\frac{1}{2}\sum_{\alpha}m^2_{S_{\alpha}}S_{\alpha}^2\,,
\end{align}
where
\begin{align}
  \left( {\mathcal{M}'}_S ^2\right)_{\alpha\beta}
=&\left( {M'}_S^2 \right)_{\alpha\beta}+\lambda^{\prime SH}_{\alpha\beta}v^2\,.
\end{align}
is diagonilized by the ortogonal matriz $\mathbf{R}$. In what follows, we assume a basis in which $\boldsymbol{\mathcal{M}}_S^2$ is already diagonal with
\begin{align*}
 \mathbf{M}_S^2=&\mathbf{R}^{\operatorname{T}} {\mathbf{M}'}_S^2\mathbf{R} \nonumber\\
\boldsymbol{\lambda}^{SH}=&  \mathbf{R}^{\operatorname{T}}\boldsymbol{\lambda}^{\prime SH} \mathbf{R}
\end{align*}
and  the conditions
\begin{align*}
  \left( {M}_S^2 \right)_{\alpha\beta}+\lambda^{SH}_{\alpha\beta}v^2=0\qquad \text{for} \qquad \alpha\ne\beta\,.
\end{align*}
the corresponding Lagrangian is
\begin{align}
\label{eq:lt13a}
  -\mathcal{L}=&M_D \epsilon_{ab}R^a_d \widetilde{R}^b_u+\tfrac{1}{2}M_N NN-h_{i\alpha} \epsilon_{ab}\widetilde{R}_u^a L_{i}^b S_{\alpha}-\lambda_d\, \epsilon_{ab}H^a R_d^b N-\lambda_u \epsilon_{ab}\widetilde{H}^a \widetilde{R}_u^b N+\text{h.c}\nonumber\\
&-\left[ \mu^2 \epsilon_{ab}\widetilde{H}^{a}H^b+\tfrac{1}{2}\lambda_1 \left( \epsilon_{ab} \widetilde{H}^{a}H^b\right)^2+\tfrac{1}{2}\left({M}_S^2\right)_{\alpha\beta} S_{\alpha}S_\beta
   +\lambda^{SH}_{\alpha\beta} \epsilon_{ab}\widetilde{H}^{a}H^bS_{\alpha}S_{\beta}+\lambda^{S}_{\alpha\beta\gamma\delta}S_{\alpha}S_{\beta}S_{\gamma}S_{\delta}  \right]
\end{align}


\section{Dirac and Majorana Fermions}

A fermion is defined to be vector-like if its left- and right-handed chiralities belongs to the same representation of
$SU(3)_C\times SU(2)_L\times U(1)_Y$. For a vector like singlet see \cite{Aoki:2011yk}. We will follow the notation of \cite{Yoshikawa:1995et}.   We now define the corresponding Dirac fermions denoted with a hat. In terms of its Weyl fermions components (without specify the undotted and dotted indices), we have
\begin{align*}
  \widehat{\psi}^-=&
  \begin{pmatrix}
   \psi_{L}^{-}\\
   \psi_{R}^{-}\\
  \end{pmatrix}
&
    \widehat{\psi}^0=&
  \begin{pmatrix}
    \psi_{L}^0\\
    \psi_{R}^0
  \end{pmatrix}
\end{align*}
moreover
\begin{align*}
  \widehat{\psi}_{(L,R)}^-=&P_{L,R}\widehat{\psi}^-&
  \widehat{\psi}_{(L,R)}^0=&P_{L,R}\widehat{\psi}^0
\end{align*}
and Dirac $SU(2)$ doublets
\begin{align*}
  \widehat{\Psi}_{(L,R)}=&P_{L,R}\widehat{\Psi}=P_{L,R}
  \begin{pmatrix}
    \widehat{\psi}^0\\
        \widehat{\psi}^-\\
  \end{pmatrix}=
  \begin{pmatrix}
    \widehat{\psi}^0_{(L,R)}\\
        \widehat{\psi}^-_{(L,R)}\\
  \end{pmatrix},&
  \overline{\widehat{\Psi}_{(L,R)}}=&  \begin{pmatrix}
    \overline{\widehat{\psi}^0}&
        \overline{\widehat{\psi}^-}\\
  \end{pmatrix}P_{R,L}=  \begin{pmatrix}
    \overline{\widehat{\psi}^0_{(L,R)}}&
        \overline{\widehat{\psi}^-_{(L,R)}}\\
  \end{pmatrix}
\end{align*}

Following the notation of \cite{Martin:2012us}
\begin{align*}
  \overline{\widehat{\psi}^-}=\left( {\widehat{\psi}^-} \right)^{\dagger}
  \begin{pmatrix}
    0 & 1\\
   1 & 0
  \end{pmatrix}=&
    \begin{pmatrix}
      \left( \psi_{R}^- \right)^{\dagger} & \left( \psi_{L}^- \right)^{\dagger}
    \end{pmatrix}&
  \overline{\widehat{\psi}^0}=\left( \widehat{\psi}^0 \right)^{\dagger}  \begin{pmatrix}
    0 & 1\\
   1 & 0
  \end{pmatrix}=&\begin{pmatrix}
{\psi_{R}^0 }^{\dagger} & {\psi_{L}^0 }^{\dagger} 
\end{pmatrix}
\end{align*}
We can now check the $SU(2)$ mass term
\begin{align}
\label{eq:mdpsipsi}
  \left( \overline{\widehat{\Psi}}_{L}\widehat{\Psi}_{R}+\overline{\widehat{\Psi}}_{R}\widehat{\Psi}_{L} \right)=&  \overline{\widehat{\Psi}}\widehat{\Psi} \nonumber\\
=&   \begin{pmatrix}
    \overline{\widehat{\psi}^0} &  \overline{\widehat{\psi}^-} 
  \end{pmatrix}
  \begin{pmatrix}
    \widehat{\psi}^0 \\
    \widehat{\psi}^-
  \end{pmatrix}\nonumber\\
= & \left(     \overline{\widehat{\psi}^0}\widehat{\psi}^0 +
    \overline{\widehat{\psi}^-} \widehat{\psi}^-
 \right) \nonumber\\
= & \left[
\begin{pmatrix}
{\psi_{R}^0 }^{\dagger} & {\psi_{L}^0 }^{\dagger} 
\end{pmatrix} \begin{pmatrix}
    \psi_{L}^0\\
    \psi_{R}^0
  \end{pmatrix}
+\begin{pmatrix}
      \left(\psi_{R}^{-}\right)^\dagger & \left(\psi_{L}^{-}\right)^\dagger
    \end{pmatrix} \begin{pmatrix}
   \psi_{L}^{-}\\
   \psi_{R}^{-}\\
  \end{pmatrix}
 \right] \nonumber\\
= & \left(
    {\psi_{R}^0 }^{\dagger}\psi_{L}^0+
   {\psi_{L}^0 }^{\dagger} \psi_{R}^0+
   \left(\psi_{R}^{-}\right)^\dagger\psi_{L}^{-}+
   \left(\psi_{L}^{-}\right)^\dagger\psi_{R}^{-}
 \right) \nonumber\\
= & \left(
    {\psi_{R}^0 }^{\dagger}\psi_{L}^0+
    \left(\psi_{R}^{-}\right)^\dagger\psi_{L}^{-}+
 \text{h.c}
 \right)\,.
\end{align}



Then
\begin{align}
\overline{\widehat{\Psi}}\widehat{\Psi} 
=& \left(\widetilde{R}_u^0 R_{d}^0-\widetilde{R}_u^{+}R_d^- +\text{h.c}  \right)  \nonumber\\
=& \left(R_d^1 \widetilde{R}_u^2-R_d^2 \widetilde{R}_u^1 +\text{h.c} \right) \nonumber\\
=& \left(\epsilon_2R_d^1 \widetilde{R}_u^2+ \epsilon_{21}R_d^2 \widetilde{R}_u^1 +\text{h.c} \right) \nonumber\\
=& \left(\epsilon_{ab}R_d^a \widetilde{R}_u^b +\text{h.c} \right)\,.
\end{align}

Since
\begin{align*}
  \widehat{e}=&
  \begin{pmatrix}
    e_L\\
    e_R
  \end{pmatrix}&
\widehat{\nu}=&
\begin{pmatrix}
\nu_L\\
0\\  
\end{pmatrix}\nonumber\\
\widehat{e}_L= P_L\widehat{e}=&
  \begin{pmatrix}
    e_L\\
    0
  \end{pmatrix}&
\widehat{\nu}_L=P_L\widehat{\nu}=&
\begin{pmatrix}
\nu_L\\
0\\  
\end{pmatrix}
\end{align*}
\begin{align*}
    \overline{\widehat{e}}=&
  \begin{pmatrix}
  e_R^{\dagger} &   e_L^{\dagger} \\
  \end{pmatrix}&
    \overline{\widehat{\nu}}=&
  \begin{pmatrix}
  0 &   \nu_L^{\dagger} \\
  \end{pmatrix}&
\end{align*}
\begin{align*}
  \widehat{L}=
  \begin{pmatrix}
  \widehat{\nu}_L\\
  \widehat{e}_L    
  \end{pmatrix}
\end{align*}
we have
\begin{align*}
  \epsilon_{ab}\widetilde{R}_{u}^a L^b S +\text{h.c}=
&\left[\widetilde{R}_u^1 L^2- \widetilde{R}_u^2 L^1 \right]S+\text{h.c}\nonumber\\
=&\left[ \widetilde{R}_u^+ e_L -\widetilde{R}_u^0 \nu_L\right]S+\text{h.c}\nonumber\\
=&-\left[ {\psi_{R}^0}^{\dagger}\nu_L  
+\left(\psi_{R}^-\right)^{\dagger} e_L    
 \right]S+\text{h.c} \nonumber\\
=&-\left[   \begin{pmatrix}
  {\psi_{R}^0}^{\dagger} &0\\
\end{pmatrix}
\begin{pmatrix}
\nu_L\\
0
\end{pmatrix}-  \begin{pmatrix}
   \left( \psi_{R}^- \right)^{\dagger} & 0
  \end{pmatrix}
  \begin{pmatrix}
    e_L\\ 
    0
  \end{pmatrix}
 \right]S +\text{h.c}\nonumber\\
=&-\overline{\widehat{\psi}^0}P_L\; P_L\widehat{\nu}S 
+\overline{\widehat{\psi}^-}P_L\;P_L\widehat{e}S
+\text{h.c}\nonumber\\
=&-\overline{\widehat{\psi}_{R}^0}\widehat{\nu}_LS
+\overline{\widehat{\psi}_{R}^-}\widehat{e}_LS
+\text{h.c}\nonumber\\
=&-\overline{\widehat{\Psi}_{R}} {\widehat{L}} S+\text{h.c}\,.
\end{align*}
If we define
\begin{align}
\label{eq:NM}
\widehat{N}=&
\begin{pmatrix}
  N & N^{\dagger}
\end{pmatrix}&
\overline{\widehat{N}}=
\begin{pmatrix}
N & N^{\dagger}   
\end{pmatrix}
\end{align}

\begin{align}
\label{eq:HRdN}
\epsilon_{ab}H^a R_d^b N+\text{h.c}=&H^1 R_d^2 N-H^2 R_d^1 N+\text{h.c}\nonumber\\
 =&H^+ R_d^- N-H^0 R_d^0 N+\text{h.c}\nonumber\\
=&-N H^0 \psi_L^0  +N H^+ \psi_{L}^- +\text{h.c}\nonumber\\
=&- \begin{pmatrix}
   N & 0
 \end{pmatrix}
H^0 
\begin{pmatrix}
  \psi_L^0\\
   0
\end{pmatrix}
+
\begin{pmatrix}
N & 0  
\end{pmatrix}
 H^+ 
  \begin{pmatrix}
\psi_{L}^-\\
   0    
  \end{pmatrix}
+\text{h.c}\nonumber\\
=&-\overline{\widehat{N}}P_L H^0 P_L\widehat{\psi}^0+\overline{\widehat{N}}P_L H^+P_L \widehat{\psi}^-+\text{h.c} \nonumber\\
=&-\overline{\widehat{N}}H^0 P_L\widehat{\psi}^0+\overline{\widehat{N}}H^+P_L \widehat{\psi}^-+\text{h.c} \nonumber\\
=&-\overline{\widehat{N}} H^0 \widehat{\psi}^0_L+\overline{\widehat{N}} H^+\widehat{\psi}^-_L +\text{h.c}\nonumber\\
=&-\overline{\widehat{N}}
\begin{pmatrix}
  H^0 & -H^{+}
\end{pmatrix}
\begin{pmatrix}
\widehat{\psi}_L^0\\
\widehat{\psi}_L^-  
\end{pmatrix}+\text{h.c}\nonumber\\
=&-\overline{\widehat{N}}\widetilde{H}^{\dagger} \widehat{\Psi}_L-\overline{\widehat{\Psi}_L}\widetilde{H} \widehat{N}\,.
\end{align}

Finally
\begin{align}
\label{eq:HRuN}
  \epsilon_{ab}\widetilde{H}^a \widetilde{R}_u^b N+\text{h.c}=&\widetilde{H}^1 \widetilde{R}_u^2 N-\widetilde{H}^2 \widetilde{R}_u^1 N +\text{h.c}\nonumber\\
=&{H^0}^* \widetilde{R}_u^0 N+{H}^-\widetilde{R}_u^+ N +\text{h.c}\nonumber\\
=&-{H^0}^* {\psi_R^0}^{\dagger} N+{H}^- \left( \psi_R^- \right)^{\dagger} N +\text{h.c}\nonumber\\
  =&-\begin{pmatrix}
{\psi_R^0}^{\dagger} & 0    
  \end{pmatrix}{H^0}^*
  \begin{pmatrix}
N\\
0    
  \end{pmatrix}
 +\begin{pmatrix}
\left( \psi_R^- \right)^{\dagger} & 0\\   
 \end{pmatrix}{H}^-
 \begin{pmatrix}
   N\\
   0
 \end{pmatrix}
 +\text{h.c}\nonumber\\
  =&-\overline{\widehat{\psi}^0}P_L{H^0}^* P_L \widehat{N} +
 \overline{\widehat{\psi}^-}P_L{H}^-P_L\widehat{N} +\text{h.c}\nonumber\\
  =&-\overline{\widehat{\psi}^0}P_L{H^0}^* \widehat{N} +
 \overline{\widehat{\psi}^-}P_L{H}^-\widehat{N} +\text{h.c}\nonumber\\
  =&-\overline{\widehat{\psi}^0_R}{H^0}^* \widehat{N} +
 \overline{\widehat{\psi}^-_{R}}{H}^-\widehat{N} +\text{h.c}\nonumber\\
  =&  \begin{pmatrix}
 \overline{\widehat{\psi}^0_R} &  \overline{\widehat{\psi}^-_{R}}
  \end{pmatrix}
  \begin{pmatrix}
{H^0}^*\\
-{H}^-    
  \end{pmatrix}
\widehat{N} +\text{h.c}\nonumber\\
=&-\overline{\widehat{\Psi}_{R}}\widetilde{H}\widehat{N} -\overline{\widehat{N}}\widetilde{H}^{\dagger}\widehat{\Psi}_R\,.
\end{align}


The Full Lagrangian for Dirac and Majorana Fermions is 
\begin{align}
\label{eq:lfull}
  -\mathcal{L}=&M_D \overline{\widehat{\Psi}}\widehat{\Psi}+\tfrac{1}{2}M_N\overline{\widehat{N}}\widehat{N}
+h_{i\alpha} \overline{\widehat{\Psi}_{R}} \widehat{L}_i S_{\alpha}
+\lambda_d\overline{\widehat{\Psi}_L}\widetilde{H} \widehat{N}
+\lambda_u\overline{\widehat{\Psi}_{R}}\widetilde{H}\widehat{N}+\text{h.c}\nonumber\\
&-\left[ \mu^2 H^{\dagger}H+\lambda_1 \left(H^{\dagger}H \right)^2+\tfrac{1}{2}\left(M_S^2\right)_{\alpha\beta} S_{\alpha}S_\beta
   +\lambda^{SH}_{\alpha\beta} H^{\dagger}H S_{\alpha}S_{\beta}+\lambda^{S}_{\alpha\beta\gamma\delta}S_{\alpha}S_{\beta}S_{\gamma}S_{\delta} \right]
\end{align}

\section{Alternative notation}
In the Lagrangian implemented in Feynrules the right-handed neutrino have implicitly the proyectors:
\begin{align}
    \mathcal{L}_A=&\left[ h_{i\alpha}\overline{\widehat{L}}\widehat{\Psi} S'_{\alpha}+\lambda_d \overline{\widehat{\Psi}^c}\left( i\sigma_2 \right) H {N}^{c}
+\lambda_u \overline{\widehat{\Psi}^c}\left( i\sigma_2 \right) H {N}+\text{h.c} \right]
+M_D\overline{\widehat{\Psi}}\widehat{\Psi}+\tfrac{1}{2}M_N\overline{\widehat{N}}\widehat{N}
\end{align}
By writing explicitly the projectors we have
\begin{align*}
    \mathcal{L}_A=&\left[ h_{i\alpha}\overline{\widehat{L}}\widehat{\Psi} S'_{\alpha}+\lambda_d \overline{\widehat{\Psi}^c}\left( i\sigma_2 \right) H P_L\widehat{N}^{c}
+\lambda_u \overline{\widehat{\Psi}^c}\left( i\sigma_2 \right) H P_R\widehat{N}+\text{h.c} \right]
+M_D\overline{\widehat{\Psi}}\widehat{\Psi}+\tfrac{1}{2}M_N\overline{\widehat{N}}\widehat{N}\
\end{align*}
We now focus in couplings with the Higgs. 
\begin{align}
 \mathcal{L}_{H} \equiv& \lambda_d \overline{\widehat{\Psi}^c}\left( -i\sigma_2^{*}  H^{*}\right)^{*} (\widehat{N}^{c})_L
+\lambda_u \overline{\widehat{\Psi}^c}\left( -i\sigma_2^{*}  H^{*}\right)^{*} \widehat{N}_R+\text{h.c} \nonumber\\
=&\lambda_d \overline{\widehat{\Psi}^c}\left( i\sigma_2  H^{*}\right)^{*} (\widehat{N}_R)^c
+\lambda_u \overline{\widehat{\Psi}^c}\left( i\sigma_2  H^{*}\right)^{*} \widehat{N}_R+\text{h.c}\nonumber\\
  =&\lambda_d \overline{\widehat{\Psi}^c} \widetilde{H}^{*} (\widehat{N}_R)^c
+\lambda_u \overline{\widehat{\Psi}^c}\widetilde{H}^{*}  \widehat{N}_R+\text{h.c}\,.
\end{align}
Taking into account that
\begin{align*}
  \overline{\widehat{\Psi}^c} \widetilde{H}^{*} (\widehat{N}_{R})^{c}=&\overline{\left[ (\widehat{N}_R)^c \right]^c} \left( \widetilde{H}^{*}  \right)^{\operatorname{T}}\left( \widehat{\Psi}^c \right)^c \nonumber\\
  \overline{\widehat{\Psi}^c} \widetilde{H}^{*} (\widehat{N}_{R})=&\overline{ (\widehat{N}_R)^c } \left( \widetilde{H}^{*}  \right)^{\operatorname{T}}\left( \widehat{\Psi}^c \right)^c \,,
\end{align*}
we have
\begin{align*}
    \mathcal{L}_H=&\lambda_d \overline{\widehat{N}_R} \left( \widetilde{H}^{*} \right)^{\operatorname{T}} \widehat{\Psi}
+\lambda_u \overline{(\widehat{N}_R)^c}\left( \widetilde{H}^{*} \right)^{\operatorname{T}}  \widehat{\Psi}+\text{h.c}\nonumber\\
  =&\lambda_d \overline{\widehat{N}_R} \widetilde{H}^{\dagger} \widehat{\Psi}
+\lambda_u \overline{(\widehat{N}_R)^c}\widetilde{H}^{\dagger} \widehat{\Psi}+\text{h.c}  \nonumber\\
  =&\lambda_d \overline{ \widehat{\Psi}} \widetilde{H}\widehat{N}_R
+\lambda_u \overline{\widehat{\Psi}} \widetilde{H} (\widehat{N}_R)^{c}+\text{h.c}  \nonumber\\
  =&\lambda_d \overline{ \widehat{\Psi}} \widetilde{H}\widehat{N}_R
+\lambda_u \overline{\widehat{\Psi}} \widetilde{H} (\widehat{N}^c)_L+\text{h.c}  \nonumber\\
  =&\lambda_d \overline{ \widehat{\Psi}} \widetilde{H}P_R\widehat{N}
+\lambda_u \overline{\widehat{\Psi}} \widetilde{H} P_L\widehat{N}^{c}+\text{h.c} \nonumber\\
  =&\lambda_d \overline{ \widehat{\Psi}_L} \widetilde{H}\widehat{N}
+\lambda_u \overline{\widehat{\Psi}_R} \widetilde{H} \widehat{N}^{c}+\text{h.c}
\end{align*}

From eq.~\eqref{eq:NM} 
\begin{align}
  \widehat{N}^{c}=&
\begin{pmatrix}
  \left( N^{\dagger} \right)^{\dagger} \\ 
  N^{\dagger} 
\end{pmatrix}+
\begin{pmatrix}
  N \\ 
  N^{\dagger} 
\end{pmatrix}=\widehat{N}
\end{align}
and we have
\begin{align}
    \mathcal{L}_A=&M_D \overline{\widehat{\Psi}}\widehat{\Psi}+\tfrac{1}{2}M_N\overline{\widehat{N}}\widehat{N}
+h_{i\alpha} \overline{\widehat{\Psi}_{R}} \widehat{L}_i S_{\alpha}
+ \lambda_d \overline{\widehat{\Psi}_L}\widetilde{H} \widehat{N}
+\lambda_u \overline{\widehat{\Psi}_{R}}\widetilde{H}\widehat{N}+\text{h.c}\,,
\end{align}
as expected from eq.~\eqref{eq:lfull}


==> preface.tex <==
\begin{preface}
	Preface goes here ...  
\end{preface}

==> summary.tex <==
The scotogenic model are ...

